Age of Information in Multi-hop Networks with Priorities

Age of Information is a new metric used in real-time status update tracking applications. It measures at the destination the time elapsed since the generation of the last received packet. In this paper, we consider the co-existence of critical and noncritical status updates in a two-hop system, for which the network assigns different scheduling priorities. Specifically, the high priority is reserved to the packets that traverse the two nodes, as they experience worse latency performance. We obtain the distribution of the age and its natural upper bound termed peak age. We provide tight upper and lower bounds for priority updates and the exact expressions for the non-critical flow of packets with a general service distribution. The results give fundamental insights for the design of age-sensitive multi-hop systems.

==> fig/Cases.tex <==
\begin{tikzpicture}[scale=0.9]

\node at (-0.4,0) {$C1$};
\draw[thick,<->] (0.0,0.2) -- (1.5,0.2);
\draw[thick,<->] (1.5,0.2) -- (3.0,0.2);
\draw[thick,<->] (3.0,0.2) -- (3.7,0.2);
\draw[ultra thick,purple,-] (0,0) -- (3,0);
\draw[ultra thick,cyan,-] (1.5,-0.15) -- (3,-0.15);
\draw[thick,<->] (0.0,-0.3) -- (1.2,-0.3);
\draw[thick,<->] (1.2,-0.3) -- (2.7,-0.3);
\node at (0.7,0.4) {$Y_{1,i}$};
\node at (2.3,0.4) {$S_{11,i}$};
\node at (3.3,0.4) {$S_{12,i}$};
\node at (0.7,-0.6) {$T_{11,i-1}$};
\node at (2,-0.6) {$T_{12,i-1}$};

\node at (4.3,0) {$C4$};
\draw[thick,<->] (4.7,0.2) -- (5.7,0.2);
\draw[thick,<->] (6.2,0.2) -- (7.7,0.2);
\draw[thick,<->] (7.7,0.2) -- (8.4,0.2);
\draw[ultra thick,purple,-] (4.7,0) -- (7.7,0);
\draw[ultra thick,cyan,-] (5.7,-0.15) -- (7.7,-0.15);
\draw[thick,<->] (4.7,-0.3) -- (6.2,-0.3);
\draw[thick,<->] (6.2,-0.3) -- (7.2,-0.3);
\node at (5.2,0.4) {$Y_{1,i}$};
\node at (7,0.4) {$S_{11,i}$};
\node at (8,0.4) {$S_{12,i}$};
\node at (5.4,-0.6) {$T_{11,i-1}$};
\node at (6.7,-0.6) {$T_{12,i-1}$};

\node at (-0.4,-1.5) {$C2$};
\draw[thick,<->] (0.0,-1.3) -- (1.5,-1.3);
\draw[thick,<->] (1.5,-1.3) -- (2.7,-1.3);
\draw[thick,<->] (3.0,-1.3) -- (3.7,-1.3);
\draw[ultra thick,purple] (0,-1.5) -- (3,-1.5);
\draw[ultra thick,cyan] (1.5,-1.65) -- (3,-1.65);
\draw[thick,<->] (0.0,-1.8) -- (1.2,-1.8);
\draw[thick,<->] (1.2,-1.8) -- (3,-1.8);
\node at (0.7,-1.1) {$Y_{1,i}$};
\node at (2.1,-1.1) {$S_{11,i}$};
\node at (3.3,-1.1) {$S_{12,i}$};
\node at (0.7,-2.1) {$T_{11,i-1}$};
\node at (2.3,-2.1) {$T_{12,i-1}$};

\node at (4.3,-1.5) {$C5$};
\draw[thick,<->] (4.7,-1.3) -- (5.7,-1.3);
\draw[thick,<->] (6.2,-1.3) -- (7.2,-1.3);
\draw[thick,<->] (7.7,-1.3) -- (8.4,-1.3);
\draw[ultra thick,purple,-] (4.7,-1.5) -- (7.7,-1.5);
\draw[ultra thick,cyan,-] (5.7,-1.65) -- (7.7,-1.65);
\draw[thick,<->] (4.7,-1.8) -- (6.2,-1.8);
\draw[thick,<->] (6.2,-1.8) -- (7.7,-1.8);
\node at (5.2,-1.1) {$Y_{1,i}$};
\node at (6.6,-1.1) {$S_{11,i}$};
\node at (8,-1.1) {$S_{12,i}$};
\node at (5.4,-2.1) {$T_{11,i-1}$};
\node at (7,-2.1) {$T_{12,i-1}$};

\node at (-0.4,-3) {$C3$};
\draw[thick,<->] (0.0,-2.8) -- (1.5,-2.8);
\draw[thick,<->] (1.5,-2.8) -- (2.7,-2.8);
\draw[thick,<->] (3.0,-2.8) -- (3.7,-2.8);
\draw[ultra thick,purple] (0,-3) -- (2.7,-3);
\draw[ultra thick,cyan] (1.5,-3.15) -- (2.7,-3.15);
\draw[thick,<->] (0.0,-3.3) -- (1.2,-3.3);
\draw[thick,<->] (1.2,-3.3) -- (2.3,-3.3);
\draw[thick,<->] (2.7,-3.3) -- (3,-3.3);
\node at (0.7,-2.6) {$Y_{1,i}$};
\node at (2.1,-2.6) {$S_{11,i}$};
\node at (3.3,-2.6) {$S_{12,i}$};
\node at (0.7,-3.6) {$T_{11,i-1}$};
\node at (2,-3.6) {$T_{12,i-1}$};
\node at (2.9,-3.6) {$\tilde{S}_{2}$};

\node at (4.3,-3) {$C6$};
\draw[thick,<->] (4.7,-2.8) -- (5.7,-2.8);
\draw[thick,<->] (6.2,-2.8) -- (7.2,-2.8);
\draw[thick,<->] (7.7,-2.8) -- (8.4,-2.8);
\draw[ultra thick,purple,-] (4.7,-3) -- (7.2,-3);
\draw[ultra thick,cyan,-] (5.7,-3.15) -- (7.2,-3.15);
\draw[thick,<->] (4.7,-3.3) -- (6.2,-3.3);
\draw[thick,<->] (6.2,-3.3) -- (6.9,-3.3);
\draw[thick,<->] (7.2,-3.3) -- (7.7,-3.3);
\node at (5.2,-2.6) {$Y_{1,i}$};
\node at (6.6,-2.6) {$S_{11,i}$};
\node at (8,-2.6) {$S_{12,i}$};
\node at (5.4,-3.6) {$T_{11,i-1}$};
\node at (6.7,-3.6) {$T_{12,i-1}$};
\node at (7.5,-3.6) {$\tilde{S}_{2}$};

\draw (2,-4.4) rectangle (6.2,-3.9);
\draw[ultra thick,purple] (3,-4.2) -- (4,-4.2);
\draw[ultra thick,cyan] (5,-4.2) -- (6,-4.2);
\node at (2.5,-4.2) {$D_{1,i}$};
\node at (4.5,-4.2) {$X_{1,i}$};

\end{tikzpicture}


==> fig/SystemModel.tex <==
\begin{tikzpicture}[scale = 0.9]
% first queue
\draw[very thick, fill=purple] (0,0) rectangle (0.4,0.8);
\draw[thin] (0.5,0) rectangle (2,0.8);
\draw[dashed, very thick, fill=purple] (1.2,0) rectangle (1.6,0.8);
\draw[fill=purple, thin] (1.6,0) rectangle (2,0.8);
\draw[thin] (2.5,0.4) circle [radius = 0.4];

% second queue
\draw[fill=purple, very thick] (4,0) rectangle (4.4,0.8);
\draw[thin] (4.5,0) rectangle (6,0.8);
\draw[fill=cyan, thin] (4.8,0) rectangle (5.2,0.8);
\draw[fill=cyan, thin] (5.2,0) rectangle (5.6,0.8);
\draw[fill=purple, dashed, very thick] (5.6,0) rectangle (6,0.8);
\draw[thin] (6.5,0.4) circle [radius = 0.4];

% the arrows and labels
\draw[thick, ->] (-1.4,0.4) -- (-0.1,0.4);
\draw[thick, ->] (0.2,0.4) -- (1.2,0.4);
\draw[thick, ->] (3,0.4) -- (3.9,0.4);
\draw[thick, ->] (4.2,0.4) -- (5.6,0.4);
\draw[thick, ->] (3,-0.1) -- (3.9,0.3);
\node at (-0.7,0.6) {$\lambda_1, \mu^{-1}$};
\node at (3.4,0.6) {$\lambda_1, b_1$};
\node at (3.5,-0.2) {$\lambda_2, b_2$};

% legend
\draw[fill=purple] (-0.5,-1) rectangle (-0.1,-0.6);
\node at (1.3,-0.8) {priority packets};
\draw[fill=cyan] (3,-1) rectangle (3.4,-0.6);
\node at (5.2,-0.8) {non-priority packets};

\end{tikzpicture}

